MobiCacher: Mobility-Aware Content Caching in Small-Cell Networks

Small-cell networks have been proposed to meet the demand of ever growing mobile data traffic. One of the prominent challenges faced by small-cell networks is the lack of sufficient backhaul capacity to connect small-cell base stations (small-BSs) to the core network. We exploit the effective application layer semantics of both spatial and temporal locality to reduce the backhaul traffic. Specifically, small-BSs are equipped with storage facility to cache contents requested by users. As the {\em cache hit ratio} increases, most of the users' requests can be satisfied locally without incurring traffic over the backhaul. To make informed caching decisions, the mobility patterns of users must be carefully considered as users might frequently migrate from one small cell to another. We study the issue of mobility-aware content caching, which is formulated into an optimization problem with the objective to maximize the caching utility. As the problem is NP-complete, we develop a polynomial-time heuristic solution termed {\em MobiCacher} with bounded approximation ratio. We also conduct trace-based simulations to evaluate the performance of {\em MobiCacher}, which show that {\em MobiCacher} yields better caching utility than existing solutions.

==> np_complete.tex <==
%% \begin{figure}
%%   \centering
%%   \includegraphics[width=.4\textwidth]{figures/3sat}
%%   \caption{An toy example of 3-SAT problem with one clause and three
%%     literals.\label{fig:toy_3sat}}
%% \end{figure}
%% 
%% In this subsection, we prove the mobility-aware small-BS caching
%% problem is NP-complete. To do so, we first cast the optimization
%% problem in Eqs.~\ref{eqn:obj}-\ref{eqn:set} as a decision problem
%% termed {\it Caching Decision Problem (CDP)}.
%% %
%% \begin{mydef}[Caching Decision Problem]
%%   %
%%   Consider a network with a set $\mathcal{F}$ of small-BSs, a set
%%   $\mathcal{I}$ of MUs, a set $\mathcal{L}$ of objects and a set
%%   $\mathcal{T}$ of consecutive time slots. A set $\mathcal{F}_i^\tau$
%%   specifies the small-BSs that are reachable from MU $i$ at time
%%   $\tau$. An MU $i$ may incur a cost $c_{i,l}$ of object $l$ if the
%%   object is not cached at a small-BS reachable from MU $i$. CDP asks
%%   whether there is a way to store objects in the caches
%%   $\{\mathcal{L}_f\}$ of small-BSs such that $|\mathcal{L}_f|\le C_f,
%%   \forall f\in\mathcal{F}$ and the total normalized costs of cached
%%   objects (defined in Eq.\ref{eqn:obj}) is larger than or equal to
%%   $K$?
%%   %
%% \end{mydef}
%% %
%% To simpify our latter discussion, we denote an instance of CDP as
%% $CDP\left(\mathcal{F}, \mathcal{I}, \mathcal{L}, \mathcal{T},
%% \{\mathcal{F}_i^\tau\}, \{C_f\}, \{c_{i,l}\}, K\right)$. It is easy to
%% see that CDP belongs to the class of NP. Our certificate is the set
%% $\mathcal{L}_f$ of objects cached at each small-BS $f$. We can easily
%% check whether any cache capacity constraint is violated and calcuate
%% the total normlized cost using Eq.~\ref{eqn:obj} to see whether the
%% cost is no smaller than $K$.
%% 
%% To show the NP-completeness, we show that the 3-CNF-SAT problem is
%% polynomial-time reducible to CDP. The 3-CNF-SAT problem
%% \cite{intro_algo} is defined as follows and is well-known to be
%% NP-complete.
%% 
%% \begin{mydef}[3-CNF-SAT]
%%   Consider a boolean formula expressed as an AND of of clauses and
%%   each clause is the OR of exactly three literals. The 3-CNF-SAT
%%   problem asks whether the boolean formula is satisfiable.
%% \end{mydef}
%% 
%% \begin{mylemma} 
%%   %
%%   3-CNF-SAT is polynomial-time reducible to CDP.
%%   %
%% \end{mylemma}
%% %
%% \begin{proof}
%%   %
%%   Consider an instance of 3-CNF-SAT, {\it i.e.}, a boolean expression
%%   of the form $\phi = C_1 \wedge C_2 \wedge \cdots \wedge C_k$ in
%%   which each clause $C$ has exactly three literals $x_C^1$, $x_C^2$
%%   and $x_C^3$. We use the notation $x\in C$ to indicate that literal
%%   $x$ appears in clause $C$. Moreover, we denote $\mathcal{C} =
%%   \left\{C_1, \cdots, C_k\right\}$ the set of all clauses in $\phi$
%%   and $\mathcal{X}$ the set of positive literals appears in $\phi$
%%   ({\it i.e.}, $\mathcal{X} = \left\{x | x \in C \mbox{ or } \neg x
%%   \in C, \exists C \in \mathcal{C}\right\}$). We construct
%%   $CDP\left(\mathcal{F}, \mathcal{I}, \mathcal{L}, \{1\},
%%   \{\mathcal{F}_i^\tau\}, \{C_f\}, \{c_{i,l}\}, K\right)$ with a
%%   single time slot as follows.
%%   %
%%   \begin{itemize}
%%     %
%%     \item For a literal $x \in \mathcal{X}$, we place both $O_x$ and
%%       $O_{\neg x}$ into $\mathcal{L}$.
%%     %
%%     \item For a literal $x \in \mathcal{X}$, we place $f_x$ with
%%       $C_{f_x} = 1$ into $\mathcal{F}$.
%%     %
%%     \item We create two sets of MUs. For a clause $C\in \mathcal{C}$,
%%       we create an MU $i_C$ and place the MU into a set
%%       $\mathcal{I}_C$. Additionaly, we create an MU $i_x$ for each
%%       literal $x \in \mathcal{X}$ and place $i_x$ into a set
%%       $\mathcal{I}_x$. Obviously $\mathcal{I} = \mathcal{I}_C \cup
%%       \mathcal{I}_x$
%%     %
%%     \item For an MU $i_C\in\mathcal{I}_C$, we connect the MU with
%%       small-BS $f_x$ if $x\in C$ or $\neg x\in C$, {\it i.e.},
%%       $\mathcal{F}^1_{i_C} = \{f_x | x\in C \mbox{ or } \neg x \in
%%     C\}$. For an MU $i_x \in \mathcal{I}_x$, we only connect it with
%%     small-BS $f_x$.
%%     %
%%     \item We now assign the normalized cost incurred by an MU to an
%%       object. For an MU $i_C\in\mathcal{I}_C$, the normalized cost is
%%       defined as
%%       %
%%       \begin{align*}
%%         %
%%         c_{i_C, O_y} = \left\{
%%           %
%%           \begin{array}{l l} %
%%             2 & \mbox{if } y \in C, \\ 
%%             %
%%             1 & \mbox{if } \neg y \in C, \\ 
%%             %
%%             0 & \mbox{otherwise}.  
%%           %
%%           \end{array}
%%           %
%%           \right.  
%%           %
%%         \end{align*}
%%       %
%%       Also, for an MU $i_x\in\mathcal{I}_x$, the normalized cost is
%%       defined as
%%       %
%%       \begin{align*}
%%         %
%%         c_{i_x, O_y} = \left\{
%%           %
%%           \begin{array}{l l} 
%%             %
%%             3|\mathcal{C}| & \mbox{if } x = y \mbox{ or } \neg x = y,
%%             \\ 
%%             %
%%             0 & \mbox{otherwise}, \end{array}
%%           %
%%           \right.  \end{align*}
%%       %
%%       where $|\mathcal{C}|$ is the number of clauses in $\phi$ and
%%       $3|\mathcal{C}|$ is much larger than $1$. Given such a cost
%%       assignment and the fact that MU $i_x$ is only connected with
%%       small-BS $f_x$, $f_x$ will only consider caching object $O_x$ or
%%       $O_{\neg x}$.
%%     %
%%     \item Finally, we let $K = 3|\mathcal{C}||\mathcal{X}| +
%%       4|\mathcal{C}|$.
%%     %
%%   \end{itemize}
%%   %
%% 
%% If the expression $\phi$ is satisfiable, we can construct a solution
%% for CDP by letting small-BS $f_x$ cache $O_x$ if $x$ is assigned true
%% in $\phi$ or $O_{\neg x}$ otherwise. The total normalized costs of the
%% cached objects can be calculated as
%% %
%% \begin{align*}
%%   \sum_{\tau\in\{1\}} \sum_{i\in\mathcal{I}} \sum_{l \in
%%     \mathcal{O}_i^\tau} c_{i,l}
%%     %
%%     & = \sum_{i\in\mathcal{I}_C} \sum_{l \in \mathcal{O}_i^1} c_{i,l}
%%     + \sum_{i\in\mathcal{I}_x} \sum_{l \in \mathcal{O}_i^1} c_{i,l} \\
%%     %
%%     & = \sum_{i\in\mathcal{I}_C} \sum_{l \in \mathcal{O}_i^1} c_{i,l}
%%     + 3|\mathcal{C}||\mathcal{X}| \\
%%     & \ge 4|\mathcal{C}| + 3|\mathcal{C}||\mathcal{X}| 
%% \end{align*}
%% 
%% Since $\phi$ is satisfied, at
%% least one literal in each clause is assigned true. 
%% \end{proof}

